LoRTA: Low Rank Tensor Adaptation of Large Language Models

Low Rank Adaptation (LoRA) is a popular Parameter Efficient Fine Tuning (PEFT) method that effectively adapts large pre-trained models for downstream tasks. LoRA parameterizes model updates using low-rank matrices at each layer, significantly reducing the number of trainable parameters and, consequently, resource requirements during fine-tuning. However, the lower bound on the number of trainable parameters remains high due to the use of the low-rank matrix model. Recent works have addressed this limitation by proposing low rank tensor parameterizations for model updates. However, they only exploit redundancy across layers, or tensorize individual matrices using ad-hoc schemes that introduce additional hyperparameters. In this work, we propose a higher-order Candecomp/Parafac (CP) decomposition, enabling a more compact and flexible representation compared to existing matrix and tensor based PEFT methods. Our experiments on Natural Language Understanding, Instruction Tuning, Preference Optimization and Protein Folding benchmarks demonstrate that our method can achieve a reduction in the number of parameters while maintaining comparable performance.

==> 00_axis.tex <==

\usetikzlibrary{3d}

% Specify parameters for drawing
\pgfmathsetmacro{\width}{5}      % Witdth of matrix entry (pixel)
\pgfmathsetmacro{\featuresep}{0} % Separation between feature slices
\pgfmathsetmacro{\nx}{3} % Image size x
\pgfmathsetmacro{\ny}{6} % Image size y
\pgfmathsetmacro{\nz}{4} 
\pgfmathsetmacro{\lx}{int(\nx-1)} % last value of x
\pgfmathsetmacro{\ly}{int(\ny-1)} % last value of y
\pgfmathsetmacro{\lz}{int(\nz-1)} % last value of z
% Begin Figure

\begin{tikzpicture}[z  = {(0.5cm,0.5cm)},
                    x  = {(0.95cm,-0.25cm)},
                    y  = {(0cm,0.9cm)},
                    scale = 0.08,
                    % scale = 2
                   ]


\pgfmathsetmacro{\zaxispos}{-(\lz*(\width+\featuresep)}

\path [draw, -stealth, thick, black, above] 
            (0,0,\zaxispos) -- ++ (\nx*\width, 0, 0) node {$d_H$};

\path [draw, -stealth, thick, black, above] 
            (0,0,\zaxispos) -- ++ (0,\ny*\width, 0) node {$d$};

\path [draw, -stealth, thick, black, above] 
            (0,0,\zaxispos) -- ++ (0, 0, -\zaxispos) node {Heads};
            
\end{tikzpicture}

==> 10_lora_old.tex <==
%!TEX root = ../../lecture_11_12_compile_presentation/lecture_11_12_presentation.tex
%!TEX root = ../../lecture_11_12_compile_handout/lecture_11_12_handout.tex

\input{\pathfigs/000_macros_for_drawing_vectors_and_matrices.tex}

\usetikzlibrary{3d}

% Specify parameters for drawing
\pgfmathsetmacro{\width}{5}      % Witdth of matrix entry (pixel)
\pgfmathsetmacro{\featuresep}{0} % Separation between feature slices
\pgfmathsetmacro{\nx}{9} % Image size x
\pgfmathsetmacro{\ny}{9} % Image size y
\pgfmathsetmacro{\nz}{5} % Number features z

% Begin Figure
\begin{tikzpicture}[z  = {(0.5cm,0.5cm)},
                    x  = {(0.95cm,-0.25cm)},
                    y  = {(0cm,0.9cm)},
                    scale = 0.08]

\pgfmathsetmacro{\lx}{int(\nx-1)} % last value of x
\pgfmathsetmacro{\ly}{int(\ny-1)} % last value of y
\pgfmathsetmacro{\lz}{int(\nz-1)} % last value of z

\begin{scope}[opacity = 0.8]

\foreach \z in {0, ..., \lz}
{
   \pgfmathsetmacro{\thecurrentcolor}{\colors[\z*5]}
   \definecolor{currentcolor}{HTML}{\thecurrentcolor}

   % Draw the matrix slices
   \foreach \y in {0, ..., \ly}
   {
      \foreach \x in {0, ..., \lx}
      {

         \pgfmathsetmacro{\colorstrength}{random(100)}         
         
         \pgfmathsetmacro{\posx}{ (\width + 0          )*\x}
         \pgfmathsetmacro{\posy}{ (\width + 0          )*\y}
         \pgfmathsetmacro{\posz}{-(\width + \featuresep)*\z}

         \path [draw, fill = currentcolor!\colorstrength] % Back
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       \width) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Left
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Bottom
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
         \path [draw, fill = currentcolor!\colorstrength] % Front
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Right
             ( \posx,   \posy,   \posz )    ++
             ( \width,  0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Top
             ( \posx,   \posy,   \posz )    ++
             ( 0,       \width,  0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
      }
   }

   % Draw the y axis vector
   \foreach \y in {0, ..., \ly}
   {
         \pgfmathsetmacro{\colorstrength}{random(100)}         
         
         \pgfmathsetmacro{\posx}{ (\width + 0          )*\nx + 1*\width }
         \pgfmathsetmacro{\posy}{ (\width + 0          )*\y}
         \pgfmathsetmacro{\posz}{-(\width + \featuresep)*\z}

         \path [draw, fill = currentcolor!\colorstrength] % Back
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       \width) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Left
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Bottom
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
         \path [draw, fill = currentcolor!\colorstrength] % Front
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Right
             ( \posx,   \posy,   \posz )    ++
             ( \width,  0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Top
             ( \posx,   \posy,   \posz )    ++
             ( 0,       \width,  0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
   }

   % Draw the x axis vector
   \foreach \x in {0, ..., \lx}
   {
         \pgfmathsetmacro{\colorstrength}{random(100)}         
         
         \pgfmathsetmacro{\posx}{ (\width + 0          )*\x}
         \pgfmathsetmacro{\posy}{ (\width + 0          )*\ny + 1*\width}
         \pgfmathsetmacro{\posz}{-(\width + \featuresep)*\z}

         \path [draw, fill = currentcolor!\colorstrength] % Back
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       \width) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Left
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Bottom
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
         \path [draw, fill = currentcolor!\colorstrength] % Front
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Right
             ( \posx,   \posy,   \posz )    ++
             ( \width,  0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Top
             ( \posx,   \posy,   \posz )    ++
             ( 0,       \width,  0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
   }

}

\end{scope}


%\pgfmathsetmacro{\zaxispos}{-(\lz*(\width+\featuresep)}
%
%\path [draw, -stealth, thick, red, above] 
%            (0,0,\zaxispos) -- ++ (\nx*\width, 0, 0) node {x};
%
%\path [draw, -stealth, thick, red, above] 
%            (0,0,\zaxispos) -- ++ (0,\ny*\width, 0) node {y};
%
%\path [draw, -stealth, thick, red, above] 
%            (0,0,\zaxispos) -- ++ (0, 0, -\zaxispos) node {z};

\end{tikzpicture}

==> 20_lorta_old.tex <==
%!TEX root = ../../lecture_11_12_compile_presentation/lecture_11_12_presentation.tex
%!TEX root = ../../lecture_11_12_compile_handout/lecture_11_12_handout.tex

\input{\pathfigs/000_macros_for_drawing_vectors_and_matrices.tex}

\usetikzlibrary{3d}

% Specify parameters for drawing
\pgfmathsetmacro{\width}{5}      % Witdth of matrix entry (pixel)
\pgfmathsetmacro{\featuresep}{0} % Separation between feature slices
\pgfmathsetmacro{\nx}{9} % Image size x
\pgfmathsetmacro{\ny}{9} % Image size y
\pgfmathsetmacro{\nz}{5} % Number features z

% Begin Figure
\begin{tikzpicture}[z  = {(0.5cm,0.5cm)},
                    x  = {(0.95cm,-0.25cm)},
                    y  = {(0cm,0.9cm)},
                    scale = 0.08]

\pgfmathsetmacro{\lx}{int(\nx-1)} % last value of x
\pgfmathsetmacro{\ly}{int(\ny-1)} % last value of y
\pgfmathsetmacro{\lz}{int(\nz-1)} % last value of z

\begin{scope}[opacity = 0.8]

\foreach \z in {0, ..., \lz}
{
   \pgfmathsetmacro{\thecurrentcolor}{\colors[5
   *\z)]}
   \definecolor{currentcolor}{HTML}{\thecurrentcolor}

   % Draw the matrix slices
   \foreach \y in {0, ..., \ly}
   {
      \foreach \x in {0, ..., \lx}
      {

         \pgfmathsetmacro{\colorstrength}{random(100)}         
         
         \pgfmathsetmacro{\posx}{ (\width + 0          )*\x}
         \pgfmathsetmacro{\posy}{ (\width + 0          )*\y}
         \pgfmathsetmacro{\posz}{-(\width + \featuresep)*\z}

         \path [draw, fill = currentcolor!\colorstrength] % Back
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       \width) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Left
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Bottom
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
         \path [draw, fill = currentcolor!\colorstrength] % Front
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Right
             ( \posx,   \posy,   \posz )    ++
             ( \width,  0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Top
             ( \posx,   \posy,   \posz )    ++
             ( 0,       \width,  0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
      }
   }
}

   \pgfmathsetmacro{\thecurrentcolor}{\colors[16]}
   \definecolor{currentcolor}{HTML}{\thecurrentcolor}

   % Draw the y axis vector
   \foreach \y in {0, ..., \ly}
   {
         \pgfmathsetmacro{\colorstrength}{random(100)}         
         
         \pgfmathsetmacro{\posx}{ (\width + 0          )*\nx - \width }
         \pgfmathsetmacro{\posy}{ (\width + 0          )*\y}
         \pgfmathsetmacro{\posz}{-(\width+1)*\lz-0.5*\width}

         \path [draw, fill = currentcolor!\colorstrength] % Back
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       \width) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Left
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Bottom
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
         \path [draw, fill = currentcolor!\colorstrength] % Front
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Right
             ( \posx,   \posy,   \posz )    ++
             ( \width,  0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Top
             ( \posx,   \posy,   \posz )    ++
             ( 0,       \width,  0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
   }

   \pgfmathsetmacro{\thecurrentcolor}{\colors[16]}
   \definecolor{currentcolor}{HTML}{\thecurrentcolor}

   % Draw the x axis vector
   \foreach \x in {0, ..., \lx}
   {
         \pgfmathsetmacro{\colorstrength}{random(100)}         
         
         \pgfmathsetmacro{\posx}{ (\width + 0          )*\x}
         \pgfmathsetmacro{\posy}{ (\width + 0.2          )*\ny }
         \pgfmathsetmacro{\posz}{-(\width)*\lz}

         \path [draw, fill = currentcolor!\colorstrength] % Back
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       \width) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Left
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Bottom
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
         \path [draw, fill = currentcolor!\colorstrength] % Front
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Right
             ( \posx,   \posy,   \posz )    ++
             ( \width,  0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Top
             ( \posx,   \posy,   \posz )    ++
             ( 0,       \width,  0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
   }

   \pgfmathsetmacro{\thecurrentcolor}{\colors[17]}
   \definecolor{currentcolor}{HTML}{\thecurrentcolor}

   % Draw the z axis vector
   \foreach \z in {0, ..., \lz}
   {
         \pgfmathsetmacro{\colorstrength}{random(100)}         
         
         \pgfmathsetmacro{\posx}{ (\width + 0          )*\nx+0.5*\width}
         \pgfmathsetmacro{\posy}{ (\width + 0          )*\ny - 1*\width}
         \pgfmathsetmacro{\posz}{-(\width + \featuresep)*\z}

         \path [draw, fill = currentcolor!\colorstrength] % Back
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       \width) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Left
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Bottom
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
         \path [draw, fill = currentcolor!\colorstrength] % Front
             ( \posx,   \posy,   \posz )    ++
             ( 0,       0,       0     ) -- ++           
             ( \width,  0,       0     ) -- ++ 
             ( 0,       \width,  0     ) --++ 
             (-\width,  0,       0     ) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Right
             ( \posx,   \posy,   \posz )    ++
             ( \width,  0,       0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( 0,       \width,  0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (0,       -\width,  0     );
         \path [draw, fill = currentcolor!\colorstrength] % Top
             ( \posx,   \posy,   \posz )    ++
             ( 0,       \width,  0     ) -- ++           
             ( 0,       0,       \width) -- ++ 
             ( \width,  0,       0     ) --++ 
             ( 0,       0,      -\width) --++ 
             (-\width,  0,       0     );
   }

\end{scope}

\iffalse
\pgfmathsetmacro{\zaxispos}{-(\lz*(\width+\featuresep)}

\path [draw, -stealth, thick, red, above] 
            (0,0,\zaxispos) -- ++ (\nx*\width, 0, 0) node {x};

\path [draw, -stealth, thick, red, above] 
            (0,0,\zaxispos) -- ++ (0,\ny*\width, 0) node {y};

\path [draw, -stealth, thick, red, above] 
            (0,0,\zaxispos) -- ++ (0, 0, -\zaxispos) node {z};
\fi
\end{tikzpicture}

==> figure_anc/000_macros_for_drawing_tensor.tex <==
%!TEX root = ../lab_2C_classification.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Variables to scale the plot. Modify \myfactor only.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\myfactor{0.85}  \def\unit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Command to draw a matrix entry.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% There are five input variables:
%    #1: The x coordinate where the entry begins
%    #2: The y coordinate where the entry begins
%    #3: The width of the entry
%    #4: The height of entry
%    #5: The color of the entry.
%
\newcommand{\entry}[5]
{
   \path[draw, thin, black, fill=#5]
        (#1, #2) -- ++( #3,   0) % Advance x
                 -- ++(  0,  #4) % Advance y
                 -- ++(-#3,   0) % Backtrack x 
                 -- ++(  0, -#4);% Backtrack y (close cycle) 
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Command to draw a vector. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% There are five input variables:
%    #1: The x coordinate where the vector begins
%    #2: The y coordinate where the vector begins
%    #3: The width of the rectangle that represents each entry
%    #4: The height of the rectangle that represents each entry
%    #5: The number of entries in the vector
%
\newcommand{\drawvector}[5]
{

   % We loop from 1 until parameter #5. This is where the number of columns is specified

   \foreach \x in {1,...,#5}{  

      % Define the color for the entry. Randomly chosen from \colors array

      \pgfmathsetmacro{\thecurrentcolor}{\colors[random(20)]}
      \definecolor{currentcolor}{HTML}{\thecurrentcolor}

      % Write the entry of the vector

      \entry{#1}{#2 - #4 + \x*#4}{#3}{#4}{currentcolor!70}; 

   }

}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Command to draw a row vector. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% There are five input variables:
%    #1: The x coordinate where the vector begins
%    #2: The y coordinate where the vector begins
%    #3: The width of the rectangle that represents each entry
%    #4: The height of the rectangle that represents each entry
%    #5: The number of entries in the vector
%
\newcommand{\drawrowvector}[5]
{

   % We loop from 1 until parameter #5. This is where the number of columns is specified

   \foreach \x in {1,...,#5}{  

      % Define the color for the entry. Randomly chosen from \colors array

      \pgfmathsetmacro{\thecurrentcolor}{\colors[random(20)]}
      \definecolor{currentcolor}{HTML}{\thecurrentcolor}

      % Write the entry of the vector

      \entry{#1 - #3 + \x*#3}{#2}{#3}{#4}{currentcolor!70}; 

   }

}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Command to draw a matrix. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% There are five input variables:
%    #1: The x coordinate where the matrix begins
%    #2: The y coordinate where the matrix begins
%    #3: The width of the rectangle that represents each entry
%    #4: The height of the rectangle that represents each entry
%    #5: The number of rows in the matrix
%    #6: The number of columns in the matrix
%
\newcommand{\drawmatrix}[6]
{

   % We loop from 1 until parameter #5. This is where the number of rows is specified

   \foreach \u in {1,...,#5}{  

      % We loop from 1 until parameter #6. This is where the number of rows is specified

      \foreach \v in {1,...,#6}{  

         % Define the color for the entry. Randomly chosen from \colors array

         \pgfmathsetmacro{\thecurrentcolor}{\colors[random(20)]}
         \definecolor{currentcolor}{HTML}{\thecurrentcolor}

         % Write the entry of the vector

         \entry{#1 - #3 + \v*#3}{#2 - #4 + \u*#4}{#3}{#4}{currentcolor!70}; 
      
      }

   }

}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Command to draw a matrix with a random seed. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% There are five input variables:
%    #1: The x coordinate where the matrix begins
%    #2: The y coordinate where the matrix begins
%    #3: The width of the rectangle that represents each entry
%    #4: The height of the rectangle that represents each entry
%    #5: The number of rows in the matrix
%    #6: The number of columns in the matrix
%    #7: A random seed. Not really. But it works
\newcommand{\drawmatrixseed}[7]
{

   % We loop from 1 until parameter #5. This is where the number of rows is specified

   \foreach \u in {1,...,#5}{  

      % We loop from 1 until parameter #6. This is where the number of rows is specified

      \foreach \v in {1,...,#6}{  

         % Define the color for the entry. Randomly chosen from \colors array

         \pgfmathsetmacro{\thecurrentcolor}{\colors[mod(\u*\v*#7,20)]}         
         \definecolor{currentcolor}{HTML}{\thecurrentcolor}

         % Write the entry of the vector

         \entry{#1 - #3 + \v*#3}{#2 - #4 + \u*#4}{#3}{#4}{currentcolor!70}; 
      
      }

   }

}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Command to draw a black and white matrix. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% There are five input variables:
%    #1: The x coordinate where the matrix begins
%    #2: The y coordinate where the matrix begins
%    #3: The width of the rectangle that represents each entry
%    #4: The height of the rectangle that represents each entry
%    #5: The number of rows in the matrix
%    #6: The number of columns in the matrix
%
\newcommand{\drawbwmatrix}[6]
{

   % We loop from 1 until parameter #5. This is where the number of rows is specified

   \foreach \u in {1,...,#5}{  

      % We loop from 1 until parameter #6. This is where the number of rows is specified

      \foreach \v in {1,...,#6}{  

         % Define the color for the entry. Randomly chosen from \colors array

         \pgfmathsetmacro{\thecurrentcolor}{random(60)}

         % Write the entry of the vector

         \entry{#1 - #3 + \v*#3}{#2 - #4 + \u*#4}{#3}{#4}{black!\thecurrentcolor}; 
      
      }

   }

}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Array storing the colors to be used to represent different entries
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\colors{{"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", 
             "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
             "E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", 
             "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
             "D5EAE7", "F3ELEB", "F6C4E1", "F79CD4"}} 



==> support_files/conference_import_replacement.tex <==
\usepackage{natbib}
\setcitestyle{authoryear,round,citesep={;},aysep={,},yysep={;}}

\usepackage[dvipsnames]{xcolor}

==> support_files/named_comments.tex <==
% NOT-ANON
% This file contains anonymity-breaking details like author names

% ------------ Person-tagged comments
\newcommand{\ignacio}[1]{}%{\color{orange}[$\xi$che: #1]}
\newcommand{\Charilaos}[1]{}%{{\color{mycyan}[Charilaos: #1]}}


==> support_files/setup_script.tex <==


% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% % ------------ ICML Style
% \usepackage{icml2024_template/icml2024}
% If accepted, instead use the following line for the camera-ready submission:
% \usepackage[accepted]{icml2024_template/icml2024}

\input{support_files/conference_import_replacement}

\input{support_files/our_math_commands}

% % ------------ Links and references
% \usepackage[dvipsnames]{xcolor} % ICML style file already loads color -- Manually added dvipsnames option
% \definecolor{linkcolor}{RGB}{0,20,114} % Dark blue
% \definecolor{linkcolor}{RGB}{0,153,153}
\definecolor{linkcolor}{RGB}{0,120,130}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2024} with \usepackage[nohyperref]{icml2024} above.
\usepackage[colorlinks=true,
    linkcolor=linkcolor,
    citecolor=linkcolor,
    filecolor=linkcolor,
    urlcolor=linkcolor,
    pagebackref=true]{hyperref} 
\urlstyle{same}

\usepackage{url}

\renewcommand*\backref[1]{\ifx#1\relax \else (Cit. on p. #1) \fi}

% Cleveref must be loaded after hyperref and amsmath
\usepackage[capitalize]{cleveref}

\Crefname{algorithm}{Algo.}{Algos.}
\Crefname{theorem}{Thm.}{Thms.}
\Crefname{appendix}{Appx.}{Appx.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem*{nonumtheorem}{Theorem}

% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{remark}{Remark}

\theoremstyle{problem}
\newtheorem{problem}{Problem}


% % ------------ Our custom packages
% \usepackage{graphicx}
% \usepackage{subfigure}
\usepackage[textsize=tiny]{todonotes}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{adjustbox}

\usepackage{caption}
\usepackage{subcaption}

\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.17}
\usepackage{standalone}
\usetikzlibrary{shapes,arrows,fit,positioning, calc, decorations.markings}
% Caption comments
\definecolor{captiongray}{RGB}{100,100,100}
\newcommand{\captioncomment}[1]{{\color{captiongray} \footnotesize #1}}

\input{support_files/named_comments}

% % ------------ Table of Content for Appendix
\usepackage{minitoc}
% Make the "Part I" text invisible
\renewcommand \thepart{}
\renewcommand \partname{}


\newcommand{\graytext}[1]{{\color{gray}#1}}
\newcommand{\wip}[1]{{\color{orange}#1}}

